Encoder-Decoder Networks for Analyzing Thermal and Power Delivery Networks

Power delivery network (PDN) analysis and thermal analysis are computationally expensive tasks that are essential for successful IC design. Algorithmically, both these analyses have similar computational structure and complexity as they involve the solution to a partial differential equation of the same form. This paper converts these analyses into image-to-image and sequence-to-sequence translation tasks, which allows leveraging a class of machine learning models with an encoder-decoder-based generative (EDGe) architecture to address the time-intensive nature of these tasks. For PDN analysis, we propose two networks: (i) IREDGe: a full-chip static and dynamic IR drop predictor and (ii) EMEDGe: electromigration (EM) hotspot classifier based on input power, power grid distribution, and power pad distribution patterns. For thermal analysis, we propose ThermEDGe, a full-chip static and dynamic temperature estimator based on input power distribution patterns for thermal analysis. These networks are transferable across designs synthesized within the same technology and packing solution. The networks predict on-chip IR drop, EM hotspot locations, and temperature in milliseconds with negligibly small errors against commercial tools requiring several hours.

==> backup.tex <==
@string{comp = "IEEE Transactions on Computers"}
@string{cas = "IEEE Transactions on Circuits and Systems"}
@string{cas1 = "IEEE Transactions on Circuits and Systems I"}
@string{cas2 = "IEEE Transactions on Circuits and Systems II"}
@string{ibm = "IBM Journal of Research and Development"}
@string{ed = "IEEE Transactions on Electron Devices"}
@string{edl = "IEEE Electron Device Letters"}
@string{tvlsi = "IEEE Transactions on VLSI Systems"}
@string{cpmt = "IEEE Transactions on Components and Packaging Technologies"}
@string{tdmr = "IEEE Transactions on Devices and Materials Reliability"}
@string{solid = "IEEE Journal of Solid-State Circuits"}
@string{iccadold = "Proceedings of the IEEE International Conference on Computer-Aided Design"}
@string{iccad = "Proceedings of the IEEE/ACM International Conference on Computer-Aided Design"}
@string{dac = "Proceedings of the ACM/IEEE Design Automation Conference"}
@string{dacnew = "Proceedings of the ACM/EDAC/IEEE Design Automation Conference"}
@string{dacnewnew = "Proceedings of the ACM/ESDA/IEEE Design Automation Conference"}
@string{aspdac = "Proceedings of the Asia-South Pacific Design Automation Conference"}
@string{edac = "Proceedings of the European Design Automation Conference"}
@string{date = "Proceedings of the Design, Automation \& Test in Europe"}
@string{iscas = "Proceedings of the IEEE International Symposium on Circuits and Systems"}
@string{itc = "Proceedings of the IEEE International Test Conference"}
@string{iccd = "Proceedings of the IEEE International Conference on Computer Design"}
@string{cicc = "Proceedings of the IEEE Custom Integrated Circuits Conference"}
@string{ieeepr = "Proceedings of the IEEE"}
@string{isscc = "Proceedings of the IEEE International Solid-State Circuits	Conference"}
@string{isqed = "Proceedings of the IEEE International Symposium on Quality Electronic Design"}
@string{edl = "IEEE Electron Device Letters"}
@string{ispd = "Proceedings of the International Symposium on Physical Design"}
@string{dnt = "IEEE Design \& Test"}
@string{islped = "Proceedings of the ACM International Symposium on Low Power Electronics and Design"}
@string{iedm = "IEEE International Electronic Devices Meeting"}
@string{irps = "Proceedings of the IEEE International Reliability Physics Symposium"}
@string{isca = "Proceedings of the ACM International Symposium on Computer Architecture"}
@string{todaes = "ACM Transactions on Design Automation of Electronic Systems"}
@string{ectc = "Electronics Components and Technology Conference"}
@string{dmr = "IEEE Transactions on Device and Materials Reliability"}
@string{jep = "Journal of Electronic Packaging"}
@string{snsr = "IEEE Sensors Journal"}
@string{jap = "Journal of Applied Physics"}
@string{cambupress = "Cambridge University Press"}
@string{ivtc = "Proceedings of the IEEE Vehicular Technology Conference"}
@string{icdm = "IEEE Circuits and Devices Magazine"}
@string{apl = "Applied Physics Letters"}
@string{icsspd= "International Conference on Simulation of Semiconductor Processes and Devices"}
@string{mr="Microelectronics Reliability"}
@string{me="Microelectronics Engineering"}
@string{mj="Microelectronics Journal"} % added by Vidya for asap7nm PDK
@string{pfaic="Proceedings of the International Symposium on the Physical and Failure Analysis of Integrated Circuits"}
@string{mse="IEEE International Conference on Microelectronic Systems  Education"}
@string{iitc="IEEE International Interconnect Technology Conference"}
@string{sispad="International Conference on Simulation of Semiconductor Processes and Devices"}
@string{jmr = "Journal of Materials Research"}
@string{chmt = "IEEE Transactions on Components Hybrids and Manufacturing Technology"}
@string{vlsisym = "IEEE Symposium on VLSI Technology"}
@string{ijeds="IEEE Journal of the Electron Devices Society"}
@string{iirw="Proceedings of the IEEE International Integrated Reliability Workshop"}
@string{iclr= "The International Conference on Learning Representations "}
@string{nips="Advances in Neural Information Processing Systems"}
@string{icicml = "Proceedings of the International Conference on International Conference on Machine Learning"}
@string{vlsidat = "Proceedings of the International Symposium on VLSI Design, Automation and Test"}
@string{fnt = "Foundations and Trends in Electronic Design Automation"}
@string{tpds = "IEEE Transactions on Parallel and Distributed Systems"}


==> sec/outline.tex <==
\section{Introduction}
\begin{enumerate}
    \item One of the major challenges faced by an advanced-technology node IC designer is the overhead of large run-times of analysis tools. 
    \item Minimizing these runtimes are critical to opening doors to optimization that call these tools iteratively under the hood.
    \item Fast and accurate analysis tools that aid quick turn-around are particularly important for two critical, simulations that are performed
    several times during the design cycle:
        \begin{itemize}
        \item {\em Thermal analysis} which checks the feasibility of a placement/floorplan solution by computing on-chip temperature distributions in
        order to check for temperature hot spots.
        \item {\em Power delivery network (PDN) analysis}, which
        diagnoses the goodness and reliability of the PDN by determining voltage (IR) drops from the power pads to the gates and current densities for electromigration (EM) analysis.
        \end{itemize}  
    \item Similarity between PDN and thermal analysis problems with underlying similar differential equations. \blue{State the equation}
    \item \blueHL{Prior art: Explain and mention drawbacks of both ML and non-ML based existing techniques for these analyses.}

    \item In this work, we map the thermal and PDN analysis tasks into ML-world problems and leverage well-established image and time-based ML models to rapidly perform these analyses.
    \item The PDN analyses consists of full-chip static and transient IR drop estimation, and electromigration (EM) hotspot classification. The thermal analyses consist of both static and transient full-chip temperature estimation. 
    \item We translate the PDN analyses and static thermal analysis problems into image-to image translation tasks, and dynamic thermal analysis into a sequence-to-sequence translation task.
    \item The  inputs  to  the  thermal  analysis  problem  are  the  power/current distributions  and  the  outputs  are  the temperature  contours,  while the  inputs  for  the  PDN  analysis  task  are  power  distributions,  PDN density  maps,  and  power  bump  patterns  and  the  outputs  are  the IR  drop  contours and EM hotspot maps. 
    \item The  predicted  output  temperature  and  IR  drop contours  are  at  the  accuracy  level  of  a  million-node  ground  truth simulation.  
    \item By mapping these analyses into image-based tasks, we employ fully convolutional (FC) encoder decoder (EDGe) (Fig.~\ref{fig:enc-dec-arch}) networks for rapid and accurate thermal and PDN analyses. 
    \item \blueHL{ Explain Fig.~\ref{fig:enc-dec-arch}}
    \item Based on these concepts, this work, a culmination of a previous effort, proposes novel ML-based analyzers for full-chip static and transient temperature estimation, full-chip static and transient IR drop estimation, and EM hotspot classification. The fast inference times of these models enable thermal and PDN analysis in milliseconds as opposed to several hours using commercial tools.
    
\end{enumerate}
\begin{figure}[tb]
\centering
\includegraphics[width=0.45\textwidth]{figs/enc-dec-top.pdf}
\caption{Image-to-image translation using EDGe network.}
\label{fig:enc-dec-arch}
\vspace{-1.0em}
\end{figure}

\section{Adapting thermal and PDN analysis to ML}
\noindent
The focus of this work is on: (i) static and transient thermal analysis, (ii) static and transient IR drop analysis, and (iii) EM hotspot classification. We map each of these analyses into image-related tasks and leverage ML models that have proven to work well on image-based data. Temperature depends on the ability of the package and system to conduct heat to the ambient, and IR drop depends on off-chip (e.g.,package)  parasitics.  In  this  work,  our  focus  is  strictly  on-chip,  and both  ML models  are  trained  for  fixed  models  of  a given technology, package, and system.



\subsection{Static and transient thermal analysis}
\begin{enumerate}
    \item Background on conventional thermal analysis.
    \item Second order differential equation. For static case, \begin{math} \frac{\partial T}{\partial t} = 0\end{math} with a space discretization. The transient simulation requires both space and time discretization.
    \item FEM based solutions trade-off speed for accuracy.
    \item For the static case, the inputs are power values, obtained from a power analysis tool, and locations for each block, obtained from the layout database, as outlined in Fig.~\ref{fig:data-rep}(a) and (b). The outputs are temperature estimates in each of the elements. These are represented as static temperature contours as shown in Fig.~\ref{fig:data-rep}(g). 
    \item Therefore, the problem is inherently an \textit{image-to-image translation} task where the input is a 2D distribution of power called the power map and the output is its corresponding temperature map.
    \item We leverage U-Net-based EDGe networks to perform this task. 
    \item The transient case demands finding the temperature across the chip as a function of time and uses time varying power estimates as input. 
    the inputs are a sequence of power maps, and the output is a sequence of temperature contours.
    \item We map this analysis into a \textit{sequence-to-sequence translation} task where the input is a sequence power maps, and the output is a sequence of temperature contours.
    \item Due to the large thermal time constants, memory and time aspect in this analysis, we leverage long short term memory (LSTM)-based EDGe networks to perform this task. Further details is Section III.
\end{enumerate}

\begin{figure}[tb]
\centering
\includegraphics[width=8.8cm]{figs/data-representation.pdf}
\caption{Data representation: Mapping PDN and thermal analysis problems into
image-to-image translations tasks.}
\label{fig:data-rep}
\vspace{-2.0em}
\end{figure}


\subsection{Static and transient IR drop analysis}
\noindent
IR drop analysis amount to solving a first order differential equation of the form: 
\begin{equation}
    GV(t) + C\frac{\partial V(t)}{\partial t} = J(t) 
\end{equation}
% The static IR drop analysis task can be mapped into an image-to-image translation task where the outputs are full chip static IR drop contours (Fig.~\ref{fig:data-rep}(h)). 
where G is the conduction matrix, C is the diagonal capacitance matrix, V(t) and J(t) are vectors of voltages and currents at specific instances of time. 
In PDN analysis, on-chip PDN design, and package bump assignments impact IR drop. Therefore,
in addition to the power distributions as in the thermal analysis tasks, both static and transient IR analysis has two other inputs that must be represented as images:

\noindent
(i)~\underline{\it A PDN density map}: This feature is generated by extracting the average PDN pitch in each region of the chip. For example, when used in conjunction with the PDN styles in \cite{jsingh,OpeNPDN}, where the chip uses regionwise uniform PDNs, the average PDN density in each region, across all metal layers, is provided as an input (Fig.~\ref{fig:data-rep}(e)).

\noindent
(ii)~\underline{\it An effective distance to power pad}: This feature represents the equivalent distance from an instance to all power pads. We compute the effective distance of each instance, $d_e$, to $N$ power pads as 
$d_e^{-1} = d_1^{-1} + d_2^{-1} + ...+d_N^{-1}$
where $d_i$ is the distance of the $i^{th}$ power pad from the instance. Intuitively, the effective distance metric and the PDN density map together, represent the equivalent resistance of the path between the instance and the pad. The equivalent resistance is a parallel combination of each path. We use distance to each pad as a proxy for resistance. Fig.~\ref{fig:data-rep}(f) shows a typical ``checkerboard'' power pad layout for flip-chip packages~\cite{checkerboard1, checkerboard2}. 


Similar, to the static thermal analysis case we use U-Net-based EDGe networks to generate static IR drop estimates. However, unlike the transient thermal analysis problem, we map the transient IR drop problem into a sequence to image translation task where the sequence of images are current maps at regular time intervals.  The output image is the maximum dynamic IR drop for a given simulation time period~\cite{MAVIREC_date21, powernet}. We use a 3D U-Net based model for this task with the currents at different time steps are provided as inputs to the U-Net via different channels. 

\blue{Need to justify using U-Nets for transient IR and not LSTM networks as in transient thermal analysis.}


\subsection{EM hotspot classification}
    \begin{enumerate}
    \item Conventional EM analysis description.
    \item EM analysis generates the current density per PDN segment which we represent as an output hotspot image for each PDN layer. The image indicates EM critical and non-critical regions on the chip. Each pixel in the image represents a region of fixed size (25$\mu$m $\times$ 25$\mu$m) and a pixel is marked as critical if any segment in that region violates EM constraints. 
    \item In addition to the inputs as in IR drop analysis, since EM has an exponential dependence on temperature, we use a 2D representation of the circuit temperature as an input.
    \item Therefore, we map the EM hotspot classification into image-to-image translation similar to a segmentation problem with two classes.
    \item We use a U-Net-based model to classify each region as EM critical or not.
    \item \blue{Show an EM hotspot map in Fig.~\ref{fig:data-rep}}
    \end{enumerate}


\section{EDGe Networks for Thermal and PDN analysis}

\subsection{U-Nets for image-to-image translation}
\label{sec:unet}

\subsubsection{Overview of U-Nets}

CNNs are successful in extracting 2-D spatial information for image
classification and image labeling tasks, which have low-dimensional outputs (class or label). For PDN and thermal analysis tasks, the required outputs
are high-dimensional distributions of IR drop and temperature
contours, where the dimensionality corresponds to the number of
pixels of the image and the number of pixels 
is proportional to the size of the chip. This calls for a generator network
that can translate the extracted low-dimensional power, PDN, and effective distance to pad features from a
CNN-like encoder back into high-dimensional data representing the required output. 

\begin{figure}[htb]
\centering
\includegraphics[width=8.8cm]{figs/thermedge-arch.pdf}
\vspace{-2.5em}
\caption{U-Net-based image-to-image translation.}
\vspace{-1.0em}
\label{fig:thermedge}
\end{figure}


Fig.~\ref{fig:thermedge} shows the
structure of the EDGe network used for static thermal and PDN analysis.
It consists of two networks:

\noindent
(a)~\underline{\em Encoder/Downsampling Network} Like a CNN, the network utilizes a sequence of 2-D
convolution and max pooling layer pairs that extract key features from the
high-dimensional input feature set.  The convolution operation performs a
weighted sum on a sliding window across the image~\cite{conv-deconv}, and the
max pooling layer reduces the dimension of the input data by extracting the
maximum value from a sliding window across the input image. In
Fig.~\ref{fig:thermedge}, the feature dimension is halved at each stage by each
layer pair, and after several such operations, an encoded, low-dimensional,
compressed representation of the input data is obtained. For this reason, the
encoder is also called the downsampling path: intuitively, downsampling
helps understand the {\em ``what"} (e.g., ``Does the image contain power or IR
hotspots?'') in the input image but tends to be imprecise with the {\em ``where"}
information (e.g., the precise locations of the hotspots).  The latter is
recovered by the decoder stages.

\noindent
(b)~\underline{\em Decoder/Upsampling Network} Intuitively, the generative decoder is
responsible for retrieving the {\em ``where"} information that was lost during
downsampling, This distinguishes an EDGe network from its CNN counterpart.  The
decoder is implemented using the transpose convolution~\cite{conv-deconv} and
upsampling layers. Upsampling layers are functionally the opposite of a
pooling layer, and increase the dimension of the input data matrix by replicating rows and columns.  

\subsubsection{Use of Skip Connections}

IR drop, current densities for EM, and temperature are strongly correlated to the input power -- 
a region with high power on the chip could potentially have an IR, EM, or temperature
hotspot in its vicinity.  U-Nets~\cite{unet} utilize {\it skip} connections
between the downsampling and upsampling paths, as shown in
Fig.~\ref{fig:thermedge}.  These connections take information from one layer
and incorporate it using a {\it concatenation} layer at a deeper stage skipping intermediate layers, and appends it to the embedding
along the z-dimension.  

Skip connections combine the local power, PDN information, and power pad locations from the
downsampling path with the global power information from the upsampling path,
allowing the underlying input features to 
and directly shuttle to the layers closer to the output.  This helps recover the fine-grained ({\em ``where"}) details that are lost in the encoder network (as stated before) during upsampling in the decoder for detailed temperature and IR
drop contours. 


\subsubsection{Receptive Fields in the Encoder and Decoder Networks}

The characteristic of PDN and thermal analyses problems is that the IR drop and
temperature at each location depend on both the local and global power
information. 
%This is predominant in the thermal analysis where power dissipation in one region of the chip can significantly affect temperature in other parts of the chip due to the large heat diffusion length constants.
During convolution, by sliding averaging windows of an appropriate size
across the input power image, the network captures local spatially correlated
distributions. For capturing the larger global impact of power on temperature
and IR drop, max pooling layers are used after each convolution to
appropriately increase the size of the {\it receptive field} at each stage of
the network. The {\it receptive field} is defined as the region in the input
2-D space that affects a particular pixel, and it determines the impact
local, neighboring, and global features have on the analyses.  

In a deep network, the value of each pixel feature is
affected by all of the other pixels in the receptive field at the previous convolution stage, with the largest contributions coming from pixels near the center
of the receptive field.  Thus, each feature not only captures its receptive field in the input image, but also gives an exponentially higher weight to the middle of that region~\cite{receptive-field}. This matches
with our applications, where both thermal and IR maps for a pixel are most
affected by the features in the same pixel, and partially by features in
nearby pixels, with decreasing importance for those that are farther away.
The size of the receptive field at each stage in the network is determined by the filter sizes and the number of the convolutional and max pooling layers.


On both the encoder and decoder sides in Fig.~\ref{fig:thermedge}, we use three
stacked convolution layers, each followed by 2$\times$2 max-pooling to
extract the features from the power and PDN density images. The number of layers and filter sizes are determined based on the magnitude of the hotspot size encountered during design iterations.


\subsection{LSTM-based model for sequence-to-sequence translation}

Long short term memory (LSTM) based EDGe networks are a special kind of recurrent neural
network (RNN) that are known to be capable of learning long term dependencies
in data sequences, i.e., they have a memory component and are capable of learning
from past information in the sequence. 

\begin{figure}[h]
\centering
\includegraphics[width=0.47\textwidth]{figs/lstm-edge.pdf}
\caption{LSTM-based network for transient ThermEDGe.}
\vspace{-1.0em}
\label{fig:lstm-edge}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=8cm]{figs/conv-lstm.pdf}
\caption{Conventional (left) and ConvLSTM (right) cells.}
\label{fig:conv-lstm}
\end{figure}


For transient thermal analysis,  the structure of ThermEDGe is shown in Fig.~\ref{fig:lstm-edge}. The core architecture 
is an EDGe network, similar to the static analysis problem described in Section~\ref{sec:unet}, except that  the 
network uses additional LSTM cells to account for the time-varying component. The figure demonstrates the time-unrolled LSTM where input power
frames are passed to the network one frame at a time. The LSTM cell accounts
for the history of the power maps to generate the output temperature frames.  The network is used for  sequence-to-sequence translation in transient thermal analysis, where the input is a set of time-varying power maps and the output is a set of time-varying temperature maps (Section~\ref{sec:problem-def}).

Similar to the static ThermEDGe network (Fig.~\ref{fig:thermedge}), the encoder consists of convolution and max pooling layers to downsample and extract critical local and global spatial information and the decoder consists of upsampling and transpose convolution layers to upsample the encoded output. 
However, in addition, transient ThermEDGe has LSTM layers in both the encoder and decoder.

A standard LSTM cell is shown in Fig.~\ref{fig:conv-lstm} (left). 
% The key element is the cell state, represented by the
% horizontal line running through the top of the cell.  The state line,
% which depends on information from the previous output data, interacts with
% gates that determine how the current inputs will influence the cell state, and
% preserves a ``memory'' over the sequence.  The sigmoid layer within the gate
% outputs a value between zero and one, determining how much of the input should
% be transmitted through the gate.
While the basic LSTM cell uses fully connected layers within each gate, our application
uses a variation of an LSTM cell called a convolutional LSTM
(ConvLSTM)~\cite{conv-lstm}, shown in Fig.~\ref{fig:conv-lstm} (right).  In
this cell, the fully connected layers in each gate are replaced by convolution
layers that capture spatial information.  Thus, the LSTM-based EDGe network
obtains a spatiotemporal view that enables accurate inference.


\section{EDGe network training}
\noindent
We train the models in ThermEDGe and IREDGe to learn the temperature
and IR contours from the ``golden" commercial tool-generated or ground truth
data.  We train ThermEdge using the full physics-based thermal simulations from
the Ansys-Icepak~\cite{icepak} simulator, incorporating off-chip thermal
dynamics from package and system thermal characteristics.  IREDGe is trained
using static IR drop distribution from a PDN analyzer~\cite{pdnsim} for
various power, PDN density, and power pad distributions. 
\subsection{Generating training data}
\subsubsection{Thermal analysis}
\begin{itemize}
    \item Granularities and sizes of current maps with resolutions and storing as images of lower resolution.
    \item Commercial tool based estimates (Ansys Icepak)
    \item Number of datapoints
    \item For transient analysis, duration of simulation, time steps, regular time intervals
\end{itemize}
    
\subsubsection{IR drop analysis}
\begin{itemize}
    \item  Synthesize PDNs using OpeNPDN which uses a set of PDN templates with multiple layers and irregular densities for a 28nm technology node.
    \item IR drop estimates using PDNSim. 
    \item Number of PDN nodes.
    \item different patterns of power pad assignments.
    \item Golden data is a solution to equation (2)
    \item Number of datapoints.
    \item Granularities. 
    \item Duration of simulation, time steps number nodes in simulation.
    \item Dimensionality control: using a small window of current simulation and predicting one max dynamic IR drop value for a small window.
\end{itemize}


\subsubsection{EM hotspot classification}
\begin{itemize}
    \item Different models for each layer
    \item Golden data using PDNSim.
    \item EM limits are specified for a 28nm technology
    \item Conversion of per PDN segment current densities into EM hotspot maps
    \item Granularities of the PDN
\end{itemize}

\subsection{Model training}
For each analysis, details on all the models, hyperparameters. 
%Need to find a good condensed way of representing this.There are technically speaking there are 5 different models for EM itself one for each layer. 

\section{Evaluation of the EDGe Networks}
\subsection{Error metrics}
\begin{itemize}
    \item Metrics for thermal and PDN analysis
    \item Average error (\%)
    \item Maximum error (\%)
    \item Metrics for EM hotspot classification (F1 score, ROC, and PR curves)
\end{itemize}
\subsection{Static Thermal analysis}
\subsection{Transient Thermal analysis}
\subsection{Static IR drop analysis}
\subsection{Transient IR drop analysis}
\subsection{EM hotspot classification}
\begin{itemize}
    \item Results are on a per segment basis
    \item Conversion from image back to segment based classes
\end{itemize}






==> sec/outline_bare_bones.tex <==
\section{Introduction}
\begin{enumerate}
    \item One of the major challenges faced by an advanced-technology node IC designer is the overhead of large run-times of analysis tools. 
    \item Minimizing these runtimes are critical to opening doors to optimization that call these tools iteratively under the hood.
    \item Fast and accurate analysis tools that aid quick turn-around are particularly important for two critical, simulations that are performed
    several times during the design cycle:
        \begin{itemize}
        \item {\em Thermal analysis} which checks the feasibility of a placement/floorplan solution by computing on-chip temperature distributions in
        order to check for temperature hot spots.
        \item {\em Power delivery network (PDN) analysis}, which
        diagnoses the goodness and reliability of the PDN by determining voltage (IR) drops from the power pads to the gates and current densities for electromigration (EM) analysis.
        \end{itemize}  
    \item Similarity between PDN and thermal analysis problems with underlying similar differential equations. \blue{State the equation}
    \item \blueHL{Prior art: Explain and mention drawbacks of both ML and non-ML based existing techniques for these analyses.}

    \item In this work, we map the thermal and PDN analysis tasks into ML-world problems and leverage well-established image and time-based ML models to rapidly perform these analyses.
    \item The PDN analyses consists of full-chip static and transient IR drop estimation, and electromigration (EM) hotspot classification. The thermal analyses consist of both static and transient full-chip temperature estimation. 
    \item We translate the PDN analyses and static thermal analysis problems into image-to image translation tasks, and dynamic thermal analysis into a sequence-to-sequence translation task.
    \item The  inputs  to  the  thermal  analysis  problem  are  the  power/current distributions  and  the  outputs  are  the temperature  contours,  while the  inputs  for  the  PDN  analysis  task  are  power  distributions,  PDN density  maps,  and  power  bump  patterns  and  the  outputs  are  the IR  drop  contours and EM hotspot maps. 
    \item The  predicted  output  temperature  and  IR  drop contours  are  at  the  accuracy  level  of  a  million-node  ground  truth simulation.  
    \item By mapping these analyses into image-based tasks, we employ fully convolutional (FC) encoder decoder (EDGe) (Fig.~\ref{fig:enc-dec-arch}) networks for rapid and accurate thermal and PDN analyses. 
    \item \blueHL{ Explain Fig.~\ref{fig:enc-dec-arch}}
    \item Based on these concepts, this work, a culmination of a previous effort, proposes novel ML-based analyzers for full-chip static and transient temperature estimation, full-chip static and transient IR drop estimation, and EM hotspot classification. The fast inference times of these models enable thermal and PDN analysis in milliseconds as opposed to several hours using commercial tools.
    
\end{enumerate}
\begin{figure}[tb]
\centering
\includegraphics[width=0.45\textwidth]{figs/enc-dec-top.pdf}
\caption{Image-to-image translation using EDGe network.}
\label{fig:enc-dec-arch}
\vspace{-1.0em}
\end{figure}

\section{Adapting thermal and PDN analysis to ML}
\noindent
The focus of this work is on: (i) static and transient thermal analysis, (ii) static and transient IR drop analysis, and (iii) EM hotspot classification. We map each of these analyses into image-related tasks and leverage ML models that have proven to work well on image-based data. Temperature depends on the ability of the package and system to conduct heat to the ambient, and IR drop depends on off-chip (e.g.,package)  parasitics.  In  this  work,  our  focus  is  strictly  on-chip,  and both  ML models  are  trained  for  fixed  models  of  a given technology, package, and system.



\subsection{Static and transient thermal analysis}
\begin{enumerate}
    \item Background on conventional thermal analysis.
    \item Second order differential equation. 
    \begin{equation}
        \frac {\partial}{\partial x}\left ( k \frac{\partial T}{\partial x} \right ) + \frac {\partial}{\partial y}\left ( k \frac{\partial T}{\partial y} \right ) + q_v = \rho c_p\frac{\partial T}{\partial t} 
    \end{equation}
    For static case, \begin{math} \frac{\partial T}{\partial t} = 0\end{math} and demands only space disctrization while the transient simulation requires both space and time discretization.
    \item FEM based solutions trade-off speed for accuracy.
    \item For the static case, the inputs are power values, obtained from a power analysis tool, and locations for each block, obtained from the layout database, as outlined in Fig.~\ref{fig:data-rep}(a) and (b). The outputs are temperature estimates in each of the elements. These are represented as static temperature contours as shown in Fig.~\ref{fig:data-rep}(g). 
    \item Therefore, the problem is inherently an \textit{image-to-image translation} task where the input is a 2D distribution of power called the power map and the output is its corresponding temperature map.
    \item We leverage U-Net-based EDGe networks to perform this task. 
    \item The transient case demands finding the temperature across the chip as a function of time and uses time varying power estimates as input. 
    the inputs are a sequence of power maps, and the output is a sequence of temperature contours.
    \item We map this analysis into a \textit{sequence-to-sequence translation} task where the input is a sequence power maps, and the output is a sequence of temperature contours.
    \item Due to the large thermal time constants, memory and time aspect in this analysis, we leverage long short term memory (LSTM)-based EDGe networks to perform this task. Further details is Section III.
\end{enumerate}

\begin{figure}[tb]
\centering
\includegraphics[width=8.8cm]{figs/data-representation.pdf}
\caption{Data representation: Mapping PDN and thermal analysis problems into
image-to-image translations tasks.}
\label{fig:data-rep}
\vspace{-2.0em}
\end{figure}


\subsection{Static and transient IR drop analysis}
\noindent
IR drop analysis amount to solving a first order differential equation of the form: 
\begin{equation}
    GV(t) + C\frac{\partial V(t)}{\partial t} = J(t) 
\end{equation}
% The static IR drop analysis task can be mapped into an image-to-image translation task where the outputs are full chip static IR drop contours (Fig.~\ref{fig:data-rep}(h)). 
where G is the conduction matrix, C is the diagonal capacitance matrix, V(t) and J(t) are vectors of voltages and currents at specific instances of time. 
In PDN analysis, on-chip PDN design, and package bump assignments impact IR drop. Therefore,
in addition to the power distributions as in the thermal analysis tasks, both static and transient IR analysis has two other inputs that must be represented as images:

\noindent
(i)~\underline{\it A PDN density map}: This feature is generated by extracting the average PDN pitch in each region of the chip. For example, when used in conjunction with the PDN styles in \cite{jsingh,OpeNPDN}, where the chip uses regionwise uniform PDNs, the average PDN density in each region, across all metal layers, is provided as an input (Fig.~\ref{fig:data-rep}(e)).

\noindent
(ii)~\underline{\it An effective distance to power pad}: This feature represents the equivalent distance from an instance to all power pads. We compute the effective distance of each instance, $d_e$, to $N$ power pads as 
$d_e^{-1} = d_1^{-1} + d_2^{-1} + ...+d_N^{-1}$
where $d_i$ is the distance of the $i^{th}$ power pad from the instance. Intuitively, the effective distance metric and the PDN density map together, represent the equivalent resistance of the path between the instance and the pad. The equivalent resistance is a parallel combination of each path. We use distance to each pad as a proxy for resistance. Fig.~\ref{fig:data-rep}(f) shows a typical ``checkerboard'' power pad layout for flip-chip packages~\cite{checkerboard1, checkerboard2}. 


Similar, to the static thermal analysis case we use U-Net-based EDGe networks to generate static IR drop estimates. However, unlike the transient thermal analysis problem, we map the transient IR drop problem into a sequence to image translation task where the sequence of images are current maps at regular time intervals.  The output image is the maximum dynamic IR drop for a given simulation time period~\cite{MAVIREC_date21, powernet}. We use a 3D U-Net based model for this task with the currents at different time steps are provided as inputs to the U-Net via different channels. 

\blue{Need to justify using U-Nets for transient IR and not LSTM networks as in transient thermal analysis.}


\subsection{EM hotspot classification}
    \begin{enumerate}
    \item Conventional EM analysis description.
    \item EM analysis generates the current density per PDN segment which we represent as an output hotspot image for each PDN layer. The image indicates EM critical and non-critical regions on the chip. Each pixel in the image represents a region of fixed size (25$\mu$m $\times$ 25$\mu$m) and a pixel is marked as critical if any segment in that region violates EM constraints. 
    \item In addition to the inputs as in IR drop analysis, since EM has an exponential dependence on temperature, we use a 2D representation of the circuit temperature as an input.
    \item Therefore, we map the EM hotspot classification into image-to-image translation similar to a segmentation problem with two classes.
    \item We use a U-Net-based model to classify each region as EM critical or not.
    \item \blue{Show an EM hotspot map in Fig.~\ref{fig:data-rep}}
    \end{enumerate}


\section{EDGe Networks for Thermal and PDN analysis}
\noindent
\redHL{Identical to conference}
\subsection{U-Nets for image-to-image translation}
\label{sec:unet}

\subsubsection{Overview of U-Nets}


% \begin{figure}[htb]
% \centering
% \includegraphics[width=8.8cm]{figs/thermedge-arch.pdf}
% \vspace{-2.5em}
% \caption{U-Net-based image-to-image translation.}
% \vspace{-1.0em}
% \label{fig:thermedge}
% \end{figure}




\subsubsection{Use of Skip Connections}




\subsubsection{Receptive Fields in the Encoder and Decoder Networks}



\subsection{LSTM-based model for sequence-to-sequence translation}



% \begin{figure}[h]
% \centering
% \includegraphics[width=0.47\textwidth]{figs/lstm-edge.pdf}
% \caption{LSTM-based network for transient ThermEDGe.}
% \vspace{-1.0em}
% \label{fig:lstm-edge}
% \end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=8cm]{figs/conv-lstm.pdf}
% \caption{Conventional (left) and ConvLSTM (right) cells.}
% \label{fig:conv-lstm}
% \end{figure}



\section{EDGe network training}
\noindent
We train the models in ThermEDGe and IREDGe to learn the temperature
and IR contours from the ``golden" commercial tool-generated or ground truth
data.  We train ThermEdge using the full physics-based thermal simulations from
the Ansys-Icepak~\cite{icepak} simulator, incorporating off-chip thermal
dynamics from package and system thermal characteristics.  IREDGe is trained
using static IR drop distribution from a PDN analyzer~\cite{pdnsim} for
various power, PDN density, and power pad distributions. 
\subsection{Generating training data}
\subsubsection{Thermal analysis}
\begin{itemize}
    \item Granularities and sizes of current maps with resolutions and storing as images of lower resolution.
    \item Commercial tool based estimates (Ansys Icepak)
    \item Number of datapoints
    \item For transient analysis, duration of simulation, time steps, regular time intervals
\end{itemize}
    
\subsubsection{IR drop analysis}
\begin{itemize}
    \item  Synthesize PDNs using OpeNPDN which uses a set of PDN templates with multiple layers and irregular densities for a 28nm technology node.
    \item IR drop estimates using PDNSim. 
    \item Number of PDN nodes.
    \item different patterns of power pad assignments.
    \item Golden data is a solution to equation (2)
    \item Number of datapoints.
    \item Granularities. 
    \item Duration of simulation, time steps number nodes in simulation.
    \item Dimensionality control: using a small window of current simulation and predicting one max dynamic IR drop value for a small window.
\end{itemize}


\subsubsection{EM hotspot classification}
\begin{itemize}
    \item Different models for each layer
    \item Golden data using PDNSim.
    \item EM limits are specified for a 28nm technology
    \item Conversion of per PDN segment current densities into EM hotspot maps
    \item Granularities of the PDN
\end{itemize}

\subsection{Model training}
For each analysis, details on all the models and hyperparameters in possibly two tables. With a short description of how we train the models, runtimes. Similar to section 
%Need to find a good condensed way of representing this.There are technically speaking there are 5 different models for EM itself one for each layer. 

\section{Evaluation of the EDGe Networks}
\subsection{Error metrics}
\begin{itemize}
    \item Metrics for thermal and PDN analysis
    \item Average error (\%)
    \item Maximum error (\%)
    \item Metrics for EM hotspot classification (F1 score, ROC, and PR curves)
\end{itemize}
\subsection{Static Thermal analysis}
\subsection{Transient Thermal analysis}
\subsection{Static IR drop analysis}
\subsection{Transient IR drop analysis}
\subsection{EM hotspot classification}
\begin{itemize}
    \item Results are on a per segment basis
    \item Conversion from image back to segment based classes
\end{itemize}


\section{To do:}
- Address thermal analysis prior art 
- Explain the EM problem in better detail
- Implement PowerNet in transient mode
- ROC AUC for  M5 not looking good.
- Section IV: Add details on model training and hyper parameters


